Chats-Grid: An Iterative Retrieval Q&A Optimization Scheme Leveraging Large Model and Retrieval Enhancement Generation in smart grid

With rapid advancements in artificial intelligence, question-answering (Q&A) systems have become essential in intelligent search engines, virtual assistants, and customer service platforms. However, in dynamic domains like smart grids, conventional retrieval-augmented generation(RAG) Q&A systems face challenges such as inadequate retrieval quality, irrelevant responses, and inefficiencies in handling large-scale, real-time data streams. This paper proposes an optimized iterative retrieval-based Q&A framework called Chats-Grid tailored for smart grid environments. In the pre-retrieval phase, Chats-Grid advanced query expansion ensures comprehensive coverage of diverse data sources, including sensor readings, meter records, and control system parameters. During retrieval, Best Matching 25(BM25) sparse retrieval and BAAI General Embedding(BGE) dense retrieval in Chats-Grid are combined to process vast, heterogeneous datasets effectively. Post-retrieval, a fine-tuned large language model uses prompt engineering to assess relevance, filter irrelevant results, and reorder documents based on contextual accuracy. The model further generates precise, context-aware answers, adhering to quality criteria and employing a self-checking mechanism for enhanced reliability. Experimental results demonstrate Chats-Grid's superiority over state-of-the-art methods in fidelity, contextual recall, relevance, and accuracy by 2.37%, 2.19%, and 3.58% respectively. This framework advances smart grid management by improving decision-making and user interactions, fostering resilient and adaptive smart grid infrastructures.

==> old_ref.tex <==
@article{zhang2021poclib,
  title={{POCLib: A high-performance framework for enabling near orthogonal processing on compression}},
  author={Zhang, Feng and Zhai, Jidong and Shen, Xipeng and Mutlu, Onur and Du, Xiaoyong},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={33},
  number={2},
  pages={459--475},
  year={2022},
  publisher={IEEE}
}

@article{zhang2021tadoc,
  title={{TADOC: Text analytics directly on compression}},
  author={Zhang, Feng and Zhai, Jidong and Shen, Xipeng and Wang, Dalin and Chen, Zheng and Mutlu, Onur and Chen, Wenguang and Du, Xiaoyong},
  journal={The VLDB Journal},
  volume={30},
  number={2},
  pages={163--188},
  year={2021},
  publisher={Springer}
}

@article{zhang2018efficient,
  title={Efficient document analytics on compressed data: Method, challenges, algorithms, insights},
  author={Zhang, Feng and Zhai, Jidong and Shen, Xipeng and Mutlu, Onur and Chen, Wenguang},
  journal={Proceedings of the VLDB Endowment},
  volume={11},
  number={11},
  pages={1522--1535},
  year={2018},
  publisher={VLDB Endowment}
}

@article{pan2021exploring,
  title={{Exploring data analytics without decompression on embedded GPU systems}},
  author={Pan, Zaifeng and Zhang, Feng and Zhou, Yanliang and Zhai, Jidong and Shen, Xipeng and Mutlu, Onur and Du, Xiaoyong},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  volume={33},
  number={7},
  pages={1553--1568},
  year={2021},
  publisher={IEEE}
}

@inproceedings{zhang2022compressdb,
  title={{CompressDB: Enabling Efficient Compressed Data Direct Processing for Various Databases}},
  author={Zhang, Feng and Wan, Weitao and Zhang, Chenyang and Zhai, Jidong and Chai, Yunpeng and Li, Haixiang and Du, Xiaoyong},
  booktitle={Proceedings of the 2022 International Conference on Management of Data},
  pages={1655--1669},
  year={2022}
}


@incollection{pazzani2007content,
  title={Content-based recommendation systems},
  author={Pazzani, Michael J and Billsus, Daniel},
  booktitle={The adaptive web},
  pages={325--341},
  year={2007},
  publisher={Springer}
}

@incollection{schafer2007collaborative,
  title={Collaborative filtering recommender systems},
  author={Schafer, J Ben and Frankowski, Dan and Herlocker, Jon and Sen, Shilad},
  booktitle={The adaptive web},
  pages={291--324},
  year={2007},
  publisher={Springer}
}


@article{zhang2019deep,
  title={Deep learning based recommender system: A survey and new perspectives},
  author={Zhang, Shuai and Yao, Lina and Sun, Aixin and Tay, Yi},
  journal={ACM Computing Surveys (CSUR)},
  volume={52},
  number={1},
  pages={1--38},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@article{naumov2019deep,
  title={Deep learning recommendation model for personalization and recommendation systems},
  author={Naumov, Maxim and Mudigere, Dheevatsa and Shi, Hao-Jun Michael and Huang, Jianyu and Sundaraman, Narayanan and Park, Jongsoo and Wang, Xiaodong and Gupta, Udit and Wu, Carole-Jean and Azzolini, Alisson G and others},
  journal={arXiv preprint arXiv:1906.00091},
  year={2019}
}

@article{zhao2020distributed,
  title={Distributed hierarchical gpu parameter server for massive scale deep learning ads systems},
  author={Zhao, Weijie and Xie, Deping and Jia, Ronglai and Qian, Yulei and Ding, Ruiquan and Sun, Mingming and Li, Ping},
  journal={arXiv preprint arXiv:2003.05622},
  year={2020}
}

@article{mudigere2021softwarehardware,
  title={Software-Hardware Co-design for Fast and Scalable Training of Deep Learning Recommendation Models},
  author={Mudigere, Dheevatsa and Hao, Yuchen and Huang, Jianyu and Jia, Zhihao and Tulloch, Andrew and Sridharan, Srinivas and Liu, Xing and Ozdal, Mustafa and Nie, Jade and Park, Jongsoo and others},
  journal={arXiv preprint arXiv:2104.05158},
  year={2021}
}

@inproceedings{ke2020recnmp,
  title={Recnmp: Accelerating personalized recommendation with near-memory processing},
  author={Ke, Liu and Gupta, Udit and Cho, Benjamin Youngjae and Brooks, David and Chandra, Vikas and Diril, Utku and Firoozshahian, Amin and Hazelwood, Kim and Jia, Bill and Lee, Hsien-Hsin S and others},
  booktitle={2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA)},
  pages={790--803},
  year={2020},
  organization={IEEE}
}

@article{bruckner2009nash,
  title={Nash equilibria of static prediction games},
  author={Br{\"u}ckner, Michael and Scheffer, Tobias},
  journal={Advances in neural information processing systems},
  volume={22},
  pages={171--179},
  year={2009}
}

@inproceedings{chen2019behavior,
  title={Behavior sequence transformer for e-commerce recommendation in alibaba},
  author={Chen, Qiwei and Zhao, Huan and Li, Wei and Huang, Pipei and Ou, Wenwu},
  booktitle={Proceedings of the 1st International Workshop on Deep Learning Practice for High-Dimensional Sparse Data},
  pages={1--4},
  year={2019}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{yin2021tt,
  title={TT-Rec: Tensor Train Compression for Deep Learning Recommendation Models},
  author={Yin, Chunxing and Acun, Bilge and Wu, Carole-Jean and Liu, Xing},
  journal={Proceedings of Machine Learning and Systems},
  volume={3},
  year={2021}
}

 @misc{oldridge_2020, 
 title={Why isn't your Recommender System Training Faster on GPU? (and what can you do about it?)}, url={https://medium.com/nvidia-merlin/why-isnt-your-recommender-system-training-faster-on-gpu-and-what-can-you-do-about-it-6cb44a711ad4},
 journal={Medium}, 
 publisher={NVIDIA Merlin}, 
 author={Oldridge, Even}, 
 year={2020}, 
 month={Dec}} 
 
 
 @inproceedings{ma2020temporal,
  title={Temporal-Contextual Recommendation in Real-Time},
  author={Ma, Yifei and Narayanaswamy, Balakrishnan and Lin, Haibin and Ding, Hao},
  booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={2291--2299},
  year={2020}
}

@inproceedings{cheng2016wide,
  title={Wide \& deep learning for recommender systems},
  author={Cheng, Heng-Tze and Koc, Levent and Harmsen, Jeremiah and Shaked, Tal and Chandra, Tushar and Aradhye, Hrishi and Anderson, Glen and Corrado, Greg and Chai, Wei and Ispir, Mustafa and others},
  booktitle={Proceedings of the 1st workshop on deep learning for recommender systems},
  pages={7--10},
  year={2016}
}

@inproceedings{kwon2021tensor,
  title={Tensor casting: Co-designing algorithm-architecture for personalized recommendation training},
  author={Kwon, Youngeun and Lee, Yunjae and Rhu, Minsoo},
  booktitle={2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={235--248},
  year={2021},
  organization={IEEE}
}

@phdthesis{ebrahimzadeh2021accelerating,
  title={Accelerating recommendation system training by leveraging popular choices},
  author={Ebrahimzadeh Maboud, Yassaman},
  year={2021},
  school={University of British Columbia}
}

 
@misc{EmbeddingBag, 
 title={Pytorch\ EmbeddingBag}, 
 url={https://pytorch.org/docs/stable/generated/torch.nn.EmbeddingBag.html}, 
 journal={PyTorch},
 publisher={PyTorch}
}

@misc{kaggle, 
 title={Criteo display Ad challenge}, 
 url={https://www.kaggle.com/c/criteodisplay-ad-challenge}, 
 journal={ CriteoLabs}, 
 publisher={CriteoLabs}
}

@misc{Terabyte, 
 title={Terabyte\ click\ logs}, 
 url={https://labs.criteo.com/2013/12/downloadterabyte-click-logs}, 
 journal={ CriteoLabs}, 
 publisher={CriteoLabs}
}

@misc{Avazu, 
 title={Avazu mobile ads ctr}, 
 url={https://www.kaggle.com/c/avazu-ctr-prediction}, 
 publisher={Kaggle}
}

@misc{cublas,
  author = {Nvidia},
  title  = {Dense Linear Algebra on GPUs},
  url    = {developer.nvidia.com/cublas},
  howpublished = "\url{developer.nvidia.com/cublas}"
}

@inproceedings{rendle2010factorization,
  title={Factorization machines},
  author={Rendle, Steffen},
  booktitle={2010 IEEE International conference on data mining},
  pages={995--1000},
  year={2010},
  organization={IEEE}
}

@article{girvan2002community,
  title={Community structure in social and biological networks},
  author={Girvan, Michelle and Newman, Mark EJ},
  journal={Proceedings of the national academy of sciences},
  volume={99},
  number={12},
  pages={7821--7826},
  year={2002},
  publisher={National Acad Sciences}
}

@inproceedings{shiokawa2013fast,
  title={Fast algorithm for modularity-based graph clustering},
  author={Shiokawa, Hiroaki and Fujiwara, Yasuhiro and Onizuka, Makoto},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={27},
  number={1},
  year={2013}
}

@article{yang2020mixed,
  title={Mixed-Precision Embedding Using a Cache},
  author={Yang, Jie Amy and Huang, Jianyu and Park, Jongsoo and Tang, Ping Tak Peter and Tulloch, Andrew},
  journal={arXiv preprint arXiv:2010.11305},
  year={2020}
}


@article{wu2019wider,
  title={Wider or deeper: Revisiting the resnet model for visual recognition},
  author={Wu, Zifeng and Shen, Chunhua and Van Den Hengel, Anton},
  journal={Pattern Recognition},
  volume={90},
  pages={119--133},
  year={2019},
  publisher={Elsevier}
}


@misc{NvTabular, 
 title={Nvidia Merlin NvTabular}, 
 url={https://developer.nvidia.com/nvidia-merlin/nvtabular}, 
 journal={Nvidia}, 
 publisher={Nvidia}
}

@inproceedings{covington2016deep,
  title={Deep neural networks for youtube recommendations},
  author={Covington, Paul and Adams, Jay and Sargin, Emre},
  booktitle={Proceedings of the 10th ACM conference on recommender systems},
  pages={191--198},
  year={2016}
}

@inproceedings{okura2017embedding,
  title={Embedding-based news recommendation for millions of users},
  author={Okura, Shumpei and Tagami, Yukihiro and Ono, Shingo and Tajima, Akira},
  booktitle={Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={1933--1942},
  year={2017}
}

@article{gomez2015netflix,
  title={The netflix recommender system: Algorithms, business value, and innovation},
  author={Gomez-Uribe, Carlos A and Hunt, Neil},
  journal={ACM Transactions on Management Information Systems (TMIS)},
  volume={6},
  number={4},
  pages={1--19},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gupta2020deeprecsys,
  title={Deeprecsys: A system for optimizing end-to-end at-scale neural recommendation inference},
  author={Gupta, Udit and Hsia, Samuel and Saraph, Vikram and Wang, Xiaodong and Reagen, Brandon and Wei, Gu-Yeon and Lee, Hsien-Hsin S and Brooks, David and Wu, Carole-Jean},
  booktitle={2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA)},
  pages={982--995},
  year={2020},
  organization={IEEE}
}

@misc{nvidiainference, 
 title={Accelerating Wide \& Deep Recommender Inference on GPUs}, 
 url={https://developer.nvidia.com/blog/accelerating-wide-deep-recommender-inference-on-gpus/}, 
 journal={Nvidia}, 
 publisher={Nvidia}
}

@misc{hugectr, 
 title={Nvidia Merlin HugeCTR}, 
 url={https://developer.nvidia.com/nvidia-merlin/hugectr}, 
 journal={Nvidia}, 
 publisher={Nvidia}
}

@inproceedings{jiang2019xdl,
  title={XDL: an industrial deep learning framework for high-dimensional sparse data},
  author={Jiang, Biye and Deng, Chao and Yi, Huimin and Hu, Zelin and Zhou, Guorui and Zheng, Yang and Huang, Sui and Guo, Xinyang and Wang, Dongyue and Song, Yue and others},
  booktitle={Proceedings of the 1st International Workshop on Deep Learning Practice for High-Dimensional Sparse Data},
  pages={1--9},
  year={2019}
}

@article{lan2019albert,
  title={Albert: A lite bert for self-supervised learning of language representations},
  author={Lan, Zhenzhong and Chen, Mingda and Goodman, Sebastian and Gimpel, Kevin and Sharma, Piyush and Soricut, Radu},
  journal={arXiv preprint arXiv:1909.11942},
  year={2019}
}

@inproceedings{weinberger2009feature,
  title={Feature hashing for large scale multitask learning},
  author={Weinberger, Kilian and Dasgupta, Anirban and Langford, John and Smola, Alex and Attenberg, Josh},
  booktitle={Proceedings of the 26th annual international conference on machine learning},
  pages={1113--1120},
  year={2009}
}

@article{guan2019post,
  title={Post-training 4-bit quantization on embedding tables},
  author={Guan, Hui and Malevich, Andrey and Yang, Jiyan and Park, Jongsoo and Yuen, Hector},
  journal={arXiv preprint arXiv:1911.02079},
  year={2019}
}

@article{cao2020pretrained,
  title={Pretrained language models for dialogue generation with multiple input sources},
  author={Cao, Yu and Bi, Wei and Fang, Meng and Tao, Dacheng},
  journal={arXiv preprint arXiv:2010.07576},
  year={2020}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom B and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={arXiv preprint arXiv:2005.14165},
  year={2020}
}

@article{dean2012large,
  title={Large scale distributed deep networks},
  author={Dean, Jeffrey and Corrado, Greg S and Monga, Rajat and Chen, Kai and Devin, Matthieu and Le, Quoc V and Mao, Mark Z and Ranzato, Marc’Aurelio and Senior, Andrew and Tucker, Paul and others},
  year={2012}
}

@article{shoeybi2019megatron,
  title={Megatron-lm: Training multi-billion parameter language models using model parallelism},
  author={Shoeybi, Mohammad and Patwary, Mostofa and Puri, Raul and LeGresley, Patrick and Casper, Jared and Catanzaro, Bryan},
  journal={arXiv preprint arXiv:1909.08053},
  year={2019}
}

@article{harlap2018pipedream,
  title={Pipedream: Fast and efficient pipeline parallel dnn training},
  author={Harlap, Aaron and Narayanan, Deepak and Phanishayee, Amar and Seshadri, Vivek and Devanur, Nikhil and Ganger, Greg and Gibbons, Phil},
  journal={arXiv preprint arXiv:1806.03377},
  year={2018}
}

@article{huang2019gpipe,
  title={Gpipe: Efficient training of giant neural networks using pipeline parallelism},
  author={Huang, Yanping and Cheng, Youlong and Bapna, Ankur and Firat, Orhan and Chen, Dehao and Chen, Mia and Lee, HyoukJoong and Ngiam, Jiquan and Le, Quoc V and Wu, Yonghui and others},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={103--112},
  year={2019}
}

@article{chen2016training,
  title={Training deep nets with sublinear memory cost},
  author={Chen, Tianqi and Xu, Bing and Zhang, Chiyuan and Guestrin, Carlos},
  journal={arXiv preprint arXiv:1604.06174},
  year={2016}
}

@article{ren2021zero,
  title={Zero-offload: Democratizing billion-scale model training},
  author={Ren, Jie and Rajbhandari, Samyam and Aminabadi, Reza Yazdani and Ruwase, Olatunji and Yang, Shuangyan and Zhang, Minjia and Li, Dong and He, Yuxiong},
  journal={arXiv preprint arXiv:2101.06840},
  year={2021}
}

@inproceedings{huang2020swapadvisor,
  title={Swapadvisor: Pushing deep learning beyond the gpu memory limit via smart swapping},
  author={Huang, Chien-Chin and Jin, Gu and Li, Jinyang},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={1341--1355},
  year={2020}
}

@article{oseledets2011tensor,
  title={Tensor-train decomposition},
  author={Oseledets, Ivan V},
  journal={SIAM Journal on Scientific Computing},
  volume={33},
  number={5},
  pages={2295--2317},
  year={2011},
  publisher={SIAM}
}

@inproceedings{hrinchuk2020tensorized,
  title={Tensorized Embedding Layers},
  author={Hrinchuk, Oleksii and Khrulkov, Valentin and Mirvakhabova, Leyla and Orlova, Elena and Oseledets, Ivan},
  booktitle={Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: Findings},
  pages={4847--4860},
  year={2020}
}

@inproceedings{acun2021understanding,
  title={Understanding training efficiency of deep learning recommendation models at scale},
  author={Acun, Bilge and Murphy, Matthew and Wang, Xiaodong and Nie, Jade and Wu, Carole-Jean and Hazelwood, Kim},
  booktitle={2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={802--814},
  year={2021},
  organization={IEEE}
}

@inproceedings{kal2021space,
  title={SPACE: locality-aware processing in heterogeneous memory for personalized recommendations},
  author={Kal, Hongju and Lee, Seokmin and Ko, Gun and Ro, Won Woo},
  booktitle={2021 ACM/IEEE 48th Annual International Symposium on Computer Architecture (ISCA)},
  pages={679--691},
  year={2021},
  organization={IEEE}
}

@inproceedings{wang2018billion,
  title={Billion-scale commodity embedding for e-commerce recommendation in alibaba},
  author={Wang, Jizhe and Huang, Pipei and Zhao, Huan and Zhang, Zhibo and Zhao, Binqiang and Lee, Dik Lun},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={839--848},
  year={2018}
}

@inproceedings{hwang2020centaur,
  title={Centaur: A chiplet-based, hybrid sparse-dense accelerator for personalized recommendations},
  author={Hwang, Ranggi and Kim, Taehun and Kwon, Youngeun and Rhu, Minsoo},
  booktitle={2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA)},
  pages={968--981},
  year={2020},
  organization={IEEE}
}

@inproceedings{zhao2019aibox,
  title={Aibox: Ctr prediction model training on a single node},
  author={Zhao, Weijie and Zhang, Jingyuan and Xie, Deping and Qian, Yulei and Jia, Ronglai and Li, Ping},
  booktitle={Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
  pages={319--328},
  year={2019}
}

@article{liu2021learnable,
  title={Learnable Embedding Sizes for Recommender Systems},
  author={Liu, Siyi and Gao, Chen and Chen, Yihong and Jin, Depeng and Li, Yong},
  journal={arXiv preprint arXiv:2101.07577},
  year={2021}
}


@article{ghaemmaghami2020training,
  title={Training with multi-layer embeddings for model reduction},
  author={Ghaemmaghami, Benjamin and Deng, Zihao and Cho, Benjamin and Orshansky, Leo and Singh, Ashish Kumar and Erez, Mattan and Orshansky, Michael},
  journal={arXiv preprint arXiv:2006.05623},
  year={2020}
}


@inproceedings{arai2016rabbit,
  title={Rabbit order: Just-in-time parallel reordering for fast graph analysis},
  author={Arai, Junya and Shiokawa, Hiroaki and Yamamuro, Takeshi and Onizuka, Makoto and Iwamura, Sotetsu},
  booktitle={2016 IEEE International Parallel and Distributed Processing Symposium (IPDPS)},
  pages={22--31},
  year={2016},
  organization={IEEE}
}

@inproceedings{wang2014improving,
  title={Improving content-based and hybrid music recommendation using deep learning},
  author={Wang, Xinxi and Wang, Ye},
  booktitle={Proceedings of the 22nd ACM international conference on Multimedia},
  pages={627--636},
  year={2014}
}

@article{huang2021novel,
  title={A Novel Group Recommendation Model With Two-Stage Deep Learning},
  author={Huang, Zhenhua and Liu, Yajun and Zhan, Choujun and Lin, Chen and Cai, Weiwei and Chen, Yunwen},
  journal={IEEE Transactions on Systems, Man, and Cybernetics: Systems},
  year={2021},
  publisher={IEEE}
}

@inproceedings{zhou2019deep,
  title={Deep interest evolution network for click-through rate prediction},
  author={Zhou, Guorui and Mou, Na and Fan, Ying and Pi, Qi and Bian, Weijie and Zhou, Chang and Zhu, Xiaoqiang and Gai, Kun},
  booktitle={Proceedings of the AAAI conference on artificial intelligence},
  volume={33},
  number={01},
  pages={5941--5948},
  year={2019}
}

@article{wang2020adtt,
  title={ADTT: a highly efficient distributed tensor-train decomposition method for IIoT big data},
  author={Wang, Xiaokang and Yang, Laurence T and Wang, Yihao and Ren, Lei and Deen, M Jamal},
  journal={IEEE Transactions on Industrial Informatics},
  volume={17},
  number={3},
  pages={1573--1582},
  year={2020},
  publisher={IEEE}
}

@article{novikov2020tensor,
  title={Tensor Train Decomposition on TensorFlow (T3F).},
  author={Novikov, Alexander and Izmailov, Pavel and Khrulkov, Valentin and Figurnov, Michael and Oseledets, Ivan V},
  journal={J. Mach. Learn. Res.},
  volume={21},
  number={30},
  pages={1--7},
  year={2020}
}

@article{zhou2019novel,
  title={A novel modularity-based discrete state transition algorithm for community detection in networks},
  author={Zhou, Xiaojun and Yang, Ke and Xie, Yongfang and Yang, Chunhua and Huang, Tingwen},
  journal={Neurocomputing},
  volume={334},
  pages={89--99},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{kim2019parallax,
  title={Parallax: Sparsity-aware data parallel training of deep neural networks},
  author={Kim, Soojeong and Yu, Gyeong-In and Park, Hojin and Cho, Sungwoo and Jeong, Eunji and Ha, Hyeonmin and Lee, Sanha and Jeong, Joo Seong and Chun, Byung-Gon},
  booktitle={Proceedings of the Fourteenth EuroSys Conference 2019},
  pages={1--15},
  year={2019}
}

@inproceedings{li2014scaling,
  title={Scaling distributed machine learning with the parameter server},
  author={Li, Mu and Andersen, David G and Park, Jun Woo and Smola, Alexander J and Ahmed, Amr and Josifovski, Vanja and Long, James and Shekita, Eugene J and Su, Bor-Yiing},
  booktitle={11th USENIX Symposium on Operating Systems Design and Implementation (OSDI 14)},
  pages={583--598},
  year={2014}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}


@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{choquette2020nvidia,
  title={Nvidia a100 gpu: Performance \& innovation for gpu computing},
  author={Choquette, Jack and Gandhi, Wish},
  booktitle={2020 IEEE Hot Chips 32 Symposium (HCS)},
  pages={1--43},
  year={2020},
  organization={IEEE Computer Society}
}

@inproceedings{lui2021understanding,
  title={Understanding capacity-driven scale-out neural recommendation inference},
  author={Lui, Michael and Yetim, Yavuz and {\"O}zkan, {\"O}zg{\"u}r and Zhao, Zhuoran and Tsai, Shin-Yeh and Wu, Carole-Jean and Hempstead, Mark},
  booktitle={2021 IEEE International Symposium on Performance Analysis of Systems and Software (ISPASS)},
  pages={162--171},
  year={2021},
  organization={IEEE}
}

@inproceedings{guo2021scalefreectr,
  title={ScaleFreeCTR: MixCache-based Distributed Training System for CTR Models with Huge Embedding Table},
  author={Guo, Huifeng and Guo, Wei and Gao, Yong and Tang, Ruiming and He, Xiuqiang and Liu, Wenzhi},
  booktitle={Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={1269--1278},
  year={2021}
}

@misc{TorchRec,
  title={TorchRec},
  url={github.com/pytorch/torchrec},
  year={2022},
}

@inproceedings{tjandra2017compressing,
  title={Compressing recurrent neural network with tensor train},
  author={Tjandra, Andros and Sakti, Sakriani and Nakamura, Satoshi},
  booktitle={2017 International Joint Conference on Neural Networks (IJCNN)},
  pages={4451--4458},
  year={2017},
  organization={IEEE}
}

@article{qu2021hardware,
  title={Hardware-Enabled Efficient Data Processing with Tensor-Train Decomposition},
  author={Qu, Zheng and Deng, Lei and Wang, Bangyan and Chen, Hengnu and Lin, Jilan and Liang, Ling and Li, Guoqi and Zhang, Zheng and Xie, Yuan},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  year={2021}
}


==> sections/08_discussion.tex <==
\section{Discussion}
### Artifact Summary
The artifact contains codes and instructions needed to carry out experiments in the evaluation section of our paper, details including:
+ We run EL-Rec on Criteo Kaggle dataset from (https://figshare.com/articles/dataset/Kaggle_Display_Advertising_Challenge_dataset/5732310) on AWS p3.8xlarge instance and record the training time of one epoch and compare with the baselines (Facebook DLRM and TT-Rec) described in the paper.

+ The source code and associated scripts are available at the anonymous repository (XXXXXXXXXXXXXXXXXXXX). One can follow the instructions in the repo to verify the results in the paper. One needs to use the same hardware and software version, but this artifact is functional under more settings.

### Relevant Platform Details
+ Intel(R) Xeon(R) CPU E5-2686 v4 @ 2.30GHz with 240GB host memory, 4$\times$ NVIDIA Tesla V100 GPUs with 16 GB device memory.
+ Operating systems and versions: Ubuntu 18.04.6+.
+ Compilers and versions: NVCC-11.0, GCC-7.5.0
+ Libraries and versions: CUDA-11.0, Pytorch-1.7,1
+ Input datasets and versions: Criteo Kaggle dataset
